Achieving and Understanding Out-of-Distribution Generalization in Systematic Reasoning in Small-Scale Transformers

Out-of-distribution generalization (OODG) is a longstanding challenge for neural networks. This challenge is quite apparent in tasks with well-defined variables and rules, where explicit use of the rules could solve problems independently of the particular values of the variables, but networks tend to be tied to the range of values sampled in their training data. Large transformer-based language models have pushed the boundaries on how well neural networks can solve previously unseen problems, but their complexity and lack of clarity about the relevant content in their training data obfuscates how they achieve such robustness. As a step toward understanding how transformer-based systems generalize, we explore the question of OODG in small scale transformers trained with examples from a known distribution. Using a reasoning task based on the puzzle Sudoku, we show that OODG can occur on a complex problem if the training set includes examples sampled from the whole distribution of simpler component tasks. Successful generalization depends on carefully managing positional alignment when absolute position encoding is used, but we find that suppressing sensitivity to absolute positions overcomes this limitation. Taken together our results represent a small step toward understanding and promoting systematic generalization in transformers.

==> tables/grid.tex <==
%% Problem ID: Hidden single 28967
\begin{longtblr}[
    caption = {A 6x6 Sudoku grid},
    label = {table:grid}
]{
    rows = {1.4em, rowsep = .1pt},
    columns = {1.4em, colsep = .1pt},
    cells = {m,c},
    hline{1, 3, 5, 7} = {1.5pt, solid},
    hline{2, 4, 6} = {.5pt, solid},
    vline{1, 4, 7} = {1.5pt, solid},
    vline{2, 3, 5, 6} = {.5pt, solid}
}
    & 5 &   & 6 & 2 &   \\ 
  2 &   & 6 & 1 & 3 & 5 \\ 
    & 6 &   & 2 & 5 & 1 \\ 
  5 &   &   & 3 &   & 6 \\ 
  6 &   &   & 5 & 1 & 3 \\
    &   & 5 &   & 6 & 2 \\
\end{longtblr}
